Sensor-Type Classification in Buildings

Many sensors/meters are deployed in commercial buildings to monitor and optimize their performance. However, because sensor metadata is inconsistent across buildings, software-based solutions are tightly coupled to the sensor metadata conventions (i.e. schemas and naming) for each building. Running the same software across buildings requires significant integration effort. Metadata normalization is critical for scaling the deployment process and allows us to decouple building-specific conventions from the code written for building applications. It also allows us to deal with missing metadata. One important aspect of normalization is to differentiate sensors by the typeof phenomena being observed. In this paper, we propose a general, simple, yet effective classification scheme to differentiate sensors in buildings by type. We perform ensemble learning on data collected from over 2000 sensor streams in two buildings. Our approach is able to achieve more than 92% accuracy for classification within buildings and more than 82% accuracy for across buildings. We also introduce a method for identifying potential misclassified streams. This is important because it allows us to identify opportunities to attain more input from experts -- input that could help improve classification accuracy when ground truth is unavailable. We show that by adjusting a threshold value we are able to identify at least 30% of the misclassified instances.

==> setup.tex <==
\section{Experimental Setup}
\begin{figure}[h!]
\centering
	\includegraphics[width=0.4\textwidth]{./fig/SDH3_crop}
\caption{We collect data from 15 sensors in 5 rooms sitting on 4 different floors. This is a map of a section of the 3rd floor
in Sutardja Dai Hall.}
\label{fig:sdh}
\end{figure}

We perform an empirical study on sensor data collected from 15 sensors across 5 rooms. 
Each room has three sensors: a temperature sensor, a $CO_{2}$ sensor,  and a humidity sensor. 
The data from these is reported to an  
sMAP~\cite{smap} archiver. The data set used comes from two separate deployments: one is a deployment~\cite{Jay} lasting 
over 6 months on several floors in Sutardja Dai Hall (SDH) at UC Berkeley, where one sensor box -- which contains a thermometer, a humidity sensor
 and a $CO_{2}$ sensor -- is placed in each room. The box reports data over 6LowPAN~\cite{6lowpan} to a sMAP archiver every 
 15 seconds. The other is a long-term deployment comprised of thousands of sensors in dozens of buildings on campus. 
 We choose the portion of the SDH data set where the sensor devices, accessible via BACnet~\cite{BACnet}, report data to the archiver every few minutes. 
 Due to intermittent data loss, we pick a time span without interruption, starting in January until mid-February, 2013, for evaluation.

